Asymptotics of $d$-Dimensional Visibility

We consider the space $[0,n]^3$, imagined as a three dimensional, axis-aligned grid world partitioned into $n^3$ $1\times 1 \times 1$ unit cubes. Each cube is either considered to be empty, in which case a line of sight can pass through it, or obstructing, in which case no line of sight can pass through it. From a given position, some of these obstructing cubes block one's view of other obstructing cubes, leading to the following extremal problem: What is the largest number of obstructing cubes that can be simultaneously visible from the surface of an observer cube, over all possible choices of which cubes of $[0,n]^3$ are obstructing? We construct an example of a configuration in which $\Omega\big(n^\frac{8}{3}\big)$ obstructing cubes are visible, and generalize this to an example with $\Omega\big(n^{d-\frac{1}{d}}\big)$ visible obstructing hypercubes for dimension $d>3$. Using Fourier analytic techniques, we prove an $O\big(n^{d-\frac{1}{d}}\log n\big)$ upper bound in a reduced visibility setting.

==> Sections/hold.tex <==
\section{A lower bound for $f_d(n)$} \label{sec4}
In this section, we generalize the argument presented in section three to compute a lower bound in $d>3$ dimensions. To accomplish this, we must first extend the partially ordered set used in three dimensions to $d>3$ dimensions. We refer to the $d$ dimensional analogue of the parallelepiped as a $d$-paralleletope. As before, we split the interior of our $d$-hypercube into $p^{d-1}$ distinct $d$-paralleletopes. We then switch our focus to a singular one of these $d$-paralleletopes, which we shall simply to refer to as $\mathcal{P}$. As in three dimensions, with the ordered pair $(i,j,p)$, each such $d$-parallelepiped can be associated to a characteristic vertex on the upper hyperface of the large $d$-hypercube closest to the origin, and consequently the opposite vertex of the edge of $\mathcal{P}$ containing the origin. We let the characteristic vertex of $\mathcal{P}$ be $(t_1,t_2,t_3,\cdots, t_{d-1},p)$.



\subsection{Generalizing the Partially Ordered Set}
For each lateral edge of $\mathcal{P}$, we may consider the maximum number of $d$-hypercubes simultaneously visible from the observer. Let $E$ denote the lateral edge of $\mathcal{P}$ passing with the origin as one of its endpoints.
\begin{lemma}
Any line of sight (parallel to the lateral edges of $\mathcal{P}$) between the observer and an obstructing unit $d$-hypercube $C$, with which $E$ intersects, passes through the bottom d hyperface of $C$.
\end{lemma}
\begin{proof}

\end{proof}
It follows that we may collapse all of our possible obstructing $d$-hypercubes along $E$ into $(d-1)$-hypercubes parallel to the observer, and preserve the integrity of our lower bound. In an analogous fashion to the set derived for visibility in three dimensions, we find that the maximum possible number of unit $d$-hypercubes along $E$ simultaneously visible from the observer to be the width of the partially ordered set $S_d$, defined as follows.
\begin{definition}\label{def41}
Let $S_d$ denote the partially ordered set
$\{(at_1, at_2,\cdots, at_{d-1},-a )\mid 0\le a < p\}$
under product order.
\end{definition}
By considering the $d$-paralleletopes whose characteristic vertices are obtained by switching some subset of the $t_i$'s in $(t_1,t_2,\cdots,t_{d-1},p)$ with $p-t_i$'s, we find that, sacrificing a constant factor of $d$, we may in determining the number of obstructing hyprcubes contributed to the lower bound from $\mathcal{P}$, consider the maximum of the widths of all partially ordered sets of the form 
\begin{align*}
\{(\pm at_1, \pm at_2,\cdots, \pm at_{d-1},-a )\mid 0\le a \le p\} \tag{$\dagger$}
\end{align*}
\subsection{Bounding the Width}
In this section we find linearly independent vectors in $S_d$ with small coordinates absolute value wise size, demonstrating that one of the partially ordered sets obtained by negating some of the coordinates in $S_d$ (see $\dagger$) has width of $\Omega(p^{\tfrac{d-1}{d}})$, and that therefore, $f_d(n)$ is $\Omega(p^{d-\tfrac{1}{d}})$.

 Let $T(k,d)$ denote the size of the largest span of $k$ linearly independent elements of $S_d$. In the case of three dimensions, we proved that $T(2,3)$ is $\Omega(p^{\tfrac{2}{3}})$. We now extend the reasoning used in three dimension to prove an analogous and more general statement. 
\begin{lemma}\label{lem43}

For all $d>2$, $T(2,d)$ is $\Omega(p^\frac{2}{d})$.
\end{lemma}
\begin{proof}
The proof is analogous to that performed in three dimensions, starting with the fact that through a simple pigeonhole argument, there exists an element of $S_d$ all of whose components are at most $p^{\tfrac{d-1}{d}}$. 

We now use this fact to construct a pair of linearly independent vectors. Imagining all of the elements of $S_d$ as points inside of a $d$ dimensional hypercube, we partition this cube into $m^d$ cubes of side length $\frac{p}{m}$. We introduce the parameter $k$, letting $km^3<p$, ensuring that at least one of the cubes contains at least $k+1$ of these points. Solving for m, we see that $m<(\frac{p}{k})^{\tfrac{1}{d}}$. In an effort to construct vectors as small as possible, we take $m=(\frac{p}{k})^{\tfrac{1}{d}}$, which gives a box side length of $\frac{p}{m}=p^{\tfrac{d-1}{d}}k^{\tfrac{1}{d}}$. Let $s_1$ be the maximal coordinate of the element of $S_d$ with smallest maximal coordinate. Then we see that in order to ensure that the points are not in one single arithmetic progression, $\frac{p^\frac{d-1}{d}k^\frac{1}{d}}{s_1}<k+1$. Simplifying and taking $k$ is small as possible gives $k=\frac{p}{s_1^\frac{d}{d-1}}$. Plugging this in gives that the side length of the squares is $p^{\tfrac{d-1}{d}}k^{\tfrac{1}{d}}=\frac{p}{s_1^\frac{1}{d-1}}$.

It follows that $s_2\le \frac{p}{s_1^\frac{1}{d-1}}\rightarrow s_1s_2\le ps_1^{\tfrac{d-2}{d-1}}$. Plugging in $s_1\le p^\frac{d-1}{d}$ yields $s_1s_2\le p^{2-\frac{2}{d}}$. Finally, the antichain spanned by $s_1$ and $s_2$ is at least of size $\frac{p^2}{s_1s_2}=p^{\tfrac{2}{d}}$, as desired.
\end{proof}

We now let lemma 4.3 serve as our base case, constructing inductively antichains spanned by $2\le k<d$ vectors respectively.
\begin{lemma}\label{lem44}
For all $d>2$ and $k>2$, $T(k,d)$ is $\Omega(p^\frac{k}{d})$.
\end{lemma}
\begin{proof}

Fix $d>2$. We induct on $k$. By Lemma \ref{lem43}, the base case holds, so assume that for all $2\le r <k<d$, $T(r,d)$ is $\Omega(p^{\tfrac{r}{d}})$. It follows then that there exists a collection of $k-1$ linearly independent vectors $(s_1,s_2,\cdots, s_{k-1})\subseteq S_d$. The $\{s_i\}$ must satisfy $\frac{p^{k-1}}{s_1s_2\cdots s_{k-1}}\ge p^\frac{k-1}{d}\rightarrow s_1s_2\cdots s_{k-1} \le p^{(k-1)-\frac{k-1}{d}}$.

We now extend this collection by adding in $s_k$. As in Lemma 4.3 \cmnt{what, this is 4.3??}, we divide up the $d$ dimensional hypercube into uniformly sized cubes sufficiently large to contain all of the points within the antichain generated by the first $k-1$ $s_i$'s, and with extra room to construct $s_{k}$. We repeat the argument of 4.3, letting the cubes be of size $\frac{p}{m}$ we have that $km^{d} < p \rightarrow m = \bigg( \frac{p}{k} \bigg)^{\tfrac{1}{d}}$
So $C$, the side length of our cube, satisfies $C = k^{\tfrac{1}{d}} \cdot p^{\tfrac{d-1}{d}}$.

We now ensure that $C$ is sufficiently large for $s_{k}$ to exist by setting requiring that
\[
k > \frac{C^a}{s_1 \cdot s_2 \dots s_{k-1}} &= \frac{k^{\tfrac{k-1}{d}} \cdot p^{(k-1)-\frac{k-1}{d}}}{s_1 \cdot s_2 \dots s_{k-1}}\]
Rearranging gives
\[k > \frac{p^{\tfrac{(k-1)d-(k-1)}{d-(k-1)}}}{(s_1 \cdot s_2 \cdot \dots \cdot s_{k-1})^{\tfrac{d}{d-(k-1)}}} \]
Plugging in the value of $k$ to the left hand side of the above equation gives
$C > \frac{p^{\tfrac{(k-1)d-(k-1)}{d(d-(k-1)^2)}}}{(s_1 \cdot s_2 \cdot \dots \cdot s_(k-1))^{\tfrac{1}{d-(k-1)}}} \cdot p^{\tfrac{d-1}{d}}$. Finally, we have that
\begin{align*}
s_{k} \cdot (s_1 \cdot s_2 \cdot \dots \cdot s_{k-1}) &< p^{\tfrac{(k-1)d-(k-1)}{d(d-(k-1))}} \cdot p^{\tfrac{d-1}{d}} \cdot (s_1 \cdot s_2 \cdot \dots \cdot s_{k-1})^{\tfrac{d-k}{d-(k-1)}} \\
& < p^{\tfrac{(k-1)d-(k-1)}{d(d-(k-1))}} \cdot p^{\tfrac{d-1}{d}} \cdot p^{\tfrac{(k-1)d-(k-1)}{d} \cdot \frac{d-k}{d-(k-1)}} \\
&= p^{k - \frac{k}{d}}
\end{align*}
And thus the lower bound of the size of an $k$ dimensional antichain of our poset in $d$ dimensions is $\frac{p^k}{p^{k - \frac{k}{d}}} = p^{\tfrac{k}{d}}$. As our inductive step is complete, so too is our construction, and so we conclude that for $k,d>2$, $T(k,d)$ is $\Omega(p^{\tfrac{k}{d}})$.
\end{proof}

\begin{theorem}\label{thm41}

$f_d(n)$ is $\Omega(p^{d-\tfrac{1}{d}})$.
\end{theorem}
\begin{proof}
By Lemma \ref{lem44}, we can construct for each of the $p^{d-1}$ $d$-paralleletopes, a set of $\Omega(p^\frac{d-1}{d})$ simultaneously visible obstructions. It then follows that $f_d(n)$ is $\Omega(p^{d-1}\cdot p^{\tfrac{d-1}{d}})=\Omega(p^{d-\tfrac{1}{d}})$, as desired.
\end{proof}

==> Sections/to_do.tex <==
% To Do:
% - Polish end of section 8
% - Adjust introduction to account for modified section 8
% -
% -
% -
% -
% -
% -
% -
